Design and Analysis of Distributed State Estimation Algorithms Based on Belief Propagation and Applications in Smart Grids

We present a detailed study on application of factor graphs and the belief propagation (BP) algorithm to the power system state estimation (SE) problem. We start from the BP solution for the linear DC model, for which we provide a detailed convergence analysis. Using BP-based DC model we propose a fast real-time state estimator for the power system SE. The proposed estimator is easy to distribute and parallelize, thus alleviating computational limitations and allowing for processing measurements in real time. The presented algorithm may run as a continuous process. Using insights from the DC model, we use two different approaches to derive the BP algorithm for the non-linear model. The first method directly applies BP methodology, however, providing only approximate BP solution for the non-linear model. In the second approach, we make a key further step by providing the solution in which the BP is applied sequentially over the non-linear model, akin to what is done by the Gauss-Newton method. The resulting iterative Gauss-Newton belief propagation (GN-BP) algorithm can be interpreted as a distributed Gauss-Newton method with the same accuracy as the centralized SE.

==> first_pages/abstractsr.tex <==
\chap{Sa\v{z}etak} 
\pagestyle{empty}


Glavni rezultati ove teze su dizajn i analiza novih algoritama za re\v{s}avanje problema estimacije stanja baziranih na faktor grafovima i ``Belief Propagation" (BP) algoritmu koji se mogu primeniti kao centralizovani ili distribuirani estimatori stanja u elektroenergetskim sistemima. Na samom po\v{c}etku, definisan je postupak za re\v{s}avanje linearnog (DC) problema kori\v{s}\'{c}enjem BP algoritma. Pored samog algoritma data je analiza konvergencije i predlo\v{z}eno je re\v{s}enje za unapredenje konvergencije. Algoritam se mo\v{z}e jednostavno distribuirati i paralelizovati, te je pogodan za estimaciju stanja u realnom vremenu, pri \v{c}emu se informacije mogu prikupljati na asinhroni način, zaobilaze\'{c}i neke od postoje\'{c}ih rutina, kao npr. provera observabilnosti sistema. Pro\v{s}irenje algoritma za nelinearnu estimaciju stanja je mogu\'{c}e unutar datog modela.

Dalje se predla\v{z}e algoritam baziran na probabilisti\v{c}kim grafi\v{c}kim modelima koji je direktno primenjen na nelinearni problem estimacije stanja, \v{s}to predstavlja logi\v{c}an korak u tranziciji od linearnog ka nelinearnom modelu. Zbog nelinearnosti funkcija, izrazi za odredenu klasu poruka ne mogu se dobiti u zatvorenoj formi, zbog \v{c}ega rezultuju\'{c}i algoritam predstavlja aproksimativno re\v{s}enje. Nakon toga se predla\v{z}e distribuirani Gaus-Njutnov metod baziran na probabilisti\v{c}kim grafi\v{c}kim modelima i BP algoritmu koji posti\v{z}e istu ta\v{c}nost kao i centralizovana verzija Gaus-Njutnovog metoda za estimaciju stanja, te je dat i novi algoritam za otkrivanje nepouzdanih merenja (outliers) prilikom merenja elektri\v{c}nih veli\v{c}ina. Predstavljeni algoritam uspostavlja lokalni kriterijum za otkrivanje i identifikaciju nepouzdanih merenja, a numeri\v{c}ki je pokazano da algoritam zna\v{c}ajno pobolj\v{s}ava detekciju u odnosu na standardne metode.

